Tackling small eigen-gaps: Fine-grained eigenvector estimation and inference under heteroscedastic noise

This paper aims to address two fundamental challenges arising in eigenvector estimation and inference for a low-rank matrix from noisy observations: (1) how to estimate an unknown eigenvector when the eigen-gap (i.e. the spacing between the associated eigenvalue and the rest of the spectrum) is particularly small; (2) how to perform estimation and inference on linear functionals of an eigenvector -- a sort of "fine-grained" statistical reasoning that goes far beyond the usual $\ell_2$ analysis. We investigate how to address these challenges in a setting where the unknown $n\times n$ matrix is symmetric and the additive noise matrix contains independent (and non-symmetric) entries. Based on eigen-decomposition of the asymmetric data matrix, we propose estimation and uncertainty quantification procedures for an unknown eigenvector, which further allow us to reason about linear functionals of an unknown eigenvector. The proposed procedures and the accompanying theory enjoy several important features: (1) distribution-free (i.e. prior knowledge about the noise distributions is not needed); (2) adaptive to heteroscedastic noise; (3) minimax optimal under Gaussian noise. Along the way, we establish optimal procedures to construct confidence intervals for the unknown eigenvalues. All this is guaranteed even in the presence of a small eigen-gap (up to $O(\sqrt{n/\mathrm{poly}\log (n)})$ times smaller than the requirement in prior theory), which goes significantly beyond what generic matrix perturbation theory has to offer.

==> lower_bound.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Lower bounds and optimality}
\label{sec:lower-bounds}

Finally, in order to evaluate the optimality of our inferential procedure, we develop a fundamental lower bound on the variance of any unbiased estimator for $\bm{a}^{\top}\ustar$.  

\begin{theorem}[\textbf{Cram\'{e}r-Rao lower bound}] 
\label{thm:LowerBound-Gaussian}
	Suppose that the noise $\{\Hij\}$ are independently drawn from $\NORMAL(0,\sigma_{ij}^2)$ and that $\bm{M}^{\star}$ satisfies the incoherence condition with $\mu = o(n)$. In addition, consider any fixed  vector $\bm{a}$ obeying $|\bm{a}^\top \ustar| = o(\|\bm{a}\|_2)$. Then any unbiased estimator $\widehat{U}_{\bm{a}}(\bm{M})$ for $\bm{a}^{\top}\ustar$ satisfies
%
\begin{align}
\label{eq:var-lower-bound}
	\var\big[\,\widehat{U}_{\bm{a}}(\bm{M})\,\big] \geq \frac{(1-o(1))\sigmamin^2 \|\bm{a}\|_2^2 }{2(\lambdastar)^2} \triangleq \mathsf{CRLB}.
\end{align}
% 
\end{theorem}
\begin{proof} See Appendix \ref{sec:proof-lower-bound}. \end{proof}
%
To evaluate the effectiveness of our procedure, we start by considering the homoscedastic case where $\sigma_{ij}^2=\sigma_{\min}^2$ for all $1\leq i,j\leq n$, and suppose that $|\bm{a}^\top \ustar| = o(\|\bm{a}\|_2)$. It follows from Theorem \ref{thm:distribution-validity} and Lemma \ref{lem:va-properties} that, on an event with probability approaching one, the variance of our estimator $\widehat{u}_{\bm{a}}$ satisfies 
%
\begin{align}
	\var[\uahat] = (1+o(1)) \vastar =(1+o(1)) \frac{\sigma_{\min}^2\|\bm{a}\|_2^2}{2(\lambdastar)^2} = (1+o(1)) \, \mathsf{CRLB},
\end{align}
%
which matches the above Cram\'{e}r-Rao lower bound (including the pre-constant) in a very sharp manner. This confirms the information-theoretic optimality of our inferential procedure. When it comes to the more general heteroscedastic case where $\sigma_{\min}^2\leq \sigma_{ij}^2\leq \sigma_{\max}^2$, our results demonstrate that, with high probability, the variance of the proposed estimator $\widehat{u}_{\bm{a}}$ satisfies (in view of Theorem \ref{thm:distribution-validity} and Lemma \ref{lem:va-properties})
%
\begin{align}
	\var[\uahat] = (1+o(1)) \vastar \leq  \frac{(1+o(1))\sigma_{\max}^2}{\sigma_{\min}^2} \, \mathsf{CRLB} .
\end{align}
%
Therefore, the performance of our inferential procedure is at most within a factor of ${\sigma_{\max}^2}/{\sigma_{\min}^2}$ from the statistical limit. 







==> proof-lower-bound.tex <==
\section{Proof for the Cram\'er-Rao lower bound (Theorem~\ref{thm:LowerBound-Gaussian})}
\label{sec:proof-lower-bound}

This theorem is a direct consequence of the Cram\'{e}r-Rao lower bound. To simplify presentation,  we may as well assume that each $\sigma^2_{ij} = \sigmamin^{2}$ for all $1\leq i,j\leq n$; after all,  decreasing the magnitude of $\sigma_{ij}$ would only result in a smaller variance of the estimator. We also assume that there is an oracle informing us of $\{\bm{u}_k^{\star}\}_{k\neq l}$ and $\{\lambda_k^{\star}\}_{k\neq l}$, so that we can eliminate the influence of $\{\bm{u}_k^{\star}\}_{k\neq l}$ on the estimation accuracy. It light of this, it is sufficient to assume that the data matrix is given by
%
\[
	\bm{M} = \lambda_l^{\star} \bm{u}_l^{\star} \bm{u}_l^{\star\top} + \bm{H},
\]
%
which is statistically easier than the original rank-$r$ problem. 


\paragraph{Proof of the lower bound \eqref{eq:var-lower-bound-au}.}
Since the noise $\{\Hij\}$ are independently drawn from $\NORMAL(0,\sigma_{ij}^2)$, the probability density function $f(\Mbm)$ can be written as  
%
\begin{align*}
	f(\Mbm)=\frac{1}{(2\pi)^{n^{2}/2}}\prod_{i,j=1}^{n}\exp\left(-\frac{(M_{ij}-\lambda_{l}^{\star}u_{l,i}^{\star}u_{l,j}^{\star})^{2}}{2\sigma_{\min}^{2}}\right).
\end{align*}
%
In view of the Cram\'{e}r-Rao lower bound (e.g.~\cite[Theorem 3.3]{shao2003mathematical}), the variance of any unbiased estimator $\widehat{U}_{\bm{a}}(\Mbm)$ for $\bm{a}^{\top}\bm{u}_l^{\star}$ can be lower bounded by 
%
\begin{align}
\label{eq:schubert}
	\var\big[\,\widehat{U}_{\bm{a}}(\bm{M})\,\big] \geq \bm{a}^\top [\mathcal{I}(\bm{u}^{\star}_l)]^{-1} \bm{a},
\end{align}
where $\mathcal{I}(\bm{u}^{\star}_l) \defn \Exs \big[ \nabla_{\bm{u}^{\star}_l} \log f(M) 
	\left[ \nabla_{\bm{u}^{\star}_l} \log f(M)\right]^\top \big]$ denotes the Fisher information matrix. 


We begin by calculating the corresponding Fisher information matrix, and start with its diagonal entries. For any $1\leq i\leq n$, one has 
%
\begin{align*}
\big[\mathcal{I}(\bm{u}_{l}^{\star})\big]_{ii} & =\Exs\left[\frac{\partial}{u_{l,i}^{\star}}\log f(M)\left[\frac{\partial}{u_{l,i}^{\star}}\log f(M)\right]^{\top}\right]\\
 & ={\lambdastar_l}^{2}\Exs\left[\sum_{k=1}^{n}\frac{u_{l,k}^{\star}}{\sigmamin^{2}}(H_{ik}+H_{ki})\cdot\sum_{s=1}^{n}\frac{u_{l,s}^{\star}}{\sigmamin^{2}}(H_{is}+H_{si})\right]\\
%
 & =\frac{{\lambdastar_l}^{2}}{\sigmamin^{2}}\Big(4(u_{l,i}^{\star})^{2}+\sum_{k:k\neq i}2(u_{l,k}^{\star})^{2}\Big)\\
%
 & {=}\frac{2{\lambdastar_l}^{2}}{\sigmamin^{2}}\left(1+o(1)\right),
\end{align*}
%
	where the last identity follows from the fact $\ltwo{\ustar_l}^2 = 1$ and the incoherence assumption $(u_{l,k}^{\star})^2\leq \mu/n =o(1)$. 
With regards to the off-diagonal entries, we see that for any $i\neq j$, 
%
\begin{align*}
	\big[ \mathcal{I}(\ustar_l) \big]_{ij} 
	& =
	\Exs \left[ \frac{\partial}{u^\star_{l,i}} \log f(M) \left[\frac{\partial}{u^\star_{l,j}} \log f(M)\right]^\top \right] \\
	& = 
	{\lambdastar_l}^2 
	\Exs\left[ 
	\sum_{k=1}^n \frac{u^{\star}_{l,k}}{\sigmamin^2} (H_{ik}+ H_{ki}) \cdot 
	\sum_{s=1}^n \frac{u^{\star}_{l,s}}{\sigmamin^2} (H_{js}+ H_{sj})\right] \\
%
	&= \frac{2{\lambdastar_l}^2}{\sigmamin^2} u^{\star}_{l,i} u^{\star}_{l,j}.
\end{align*}
%
Here, the last equality follows from the observation that: the expectations vanish unless
$k = j$ and $s = i.$
Putting the above pieces together, we arrive at
%
\begin{align}
	\mathcal{I}(\ustar_l) = \frac{2{\lambdastar}^2}{\sigmamin^2} 
	\left( (1+ o(1))\Ind + \ustar_l {\ustar_l}^{\top} \right).
\end{align}


Further, the Woodbury matrix inversion formula tells us that
%
\begin{align}
	\big( \mathcal{I}(\ustar_l) \big)^{-1} = \frac{\sigmamin^2}{2{\lambdastar_l}^2} 
	\left( (1- o(1))\Ind - (0.5+o(1)) \ustar_l {\ustar_l}^{\top} \right) .
\end{align}
%
Therefore, the right-hand side of the expression~\eqref{eq:schubert} satisfies 
%
\begin{align}
\label{eq:symphony-great}
	\bm{a}^\top [\mathcal{I}(\ustar)]^{-1} \bm{a}
	= \frac{(1-o(1))\sigmamin^2}{2{\lambdastar_l}^2}  \left(\ltwo{\bm{a}}^2 - (\bm{a}^\top \ustar)^2 \right) 
	= \frac{(1-o(1))\sigmamin^2}{2{\lambdastar_l}^2} \|\bm{a}_l^{\perp}\|_2^2  ,
\end{align}
%
where the last equality follows since $\bm{a}_l^{\perp} = \bm{a} - (\bm{a}^{\top}\bm{u}_l^{\star}) \bm{u}_l^{\star}$ is the projection of $\bm{a}$ onto the subspace perpendicular to $\bm{u}_l^{\star}$ and hence 
$\|\bm{a}_{l}^{\perp}\|_{2}^{2}=\|\bm{a}\|_{2}^{2}-(\bm{a}^{\top}\bm{u}_{l}^{\star})^{2}$. Substitution into \eqref{eq:schubert} concludes the proof of the claim \eqref{eq:var-lower-bound-au}. 


\paragraph{Proof of the lower bound \eqref{eq:var-lower-bound-lambda}.} Suppose that an oracle informs us of the eigenvector $\bm{u}_l^{\star}$. Armed with this extra information, all of the observed data $\{M_{ij}\}_{1\leq i,j\leq n}$ can be viewed as linear measurements of $\lambda_l^{\star}$ corrupted by i.i.d.~Gaussian noise $\mathcal{N}(0,\sigma_{\min}^2)$. Using standard linear regression results \cite{lee-regression}, we know that the problem can be simplified to estimating $\lambda_l^{\star}$ from
%
\begin{align}
	y & = \langle  \bm{u}_l^{\star} \bm{u}_l^{\star\top}, \bm{u}_l^{\star} \bm{u}_l^{\star\top}   \rangle \lambda_l^{\star} + \langle \bm{H}, \bm{u}_l^{\star} \bm{u}_l^{\star\top} \rangle =\lambda_l^{\star} + Z,
\end{align}
%
where $Z\sim \mathcal{N}(0,\sigma^2_{\min})$. In view of standard lower bounds for linear regression under Gaussian noise \cite{lee-regression}, we conclude that $\mathsf{Var}(\widehat{\Lambda}(\bm{M}))\geq \sigma_{\min}^{2}$ as claimed. 





==> proof-theorem-rankr-CI.tex <==

\subsection{Proof of Theorem~\ref{thm:distribution-validity-rankr} (Old proofs)}
%\label{sec:proof-thm-distribution-validity-rankr}


\subsubsection{Distributional theory for linear forms of eigenvectors}

By virtue of Theorem \ref{thm:eigengap-condition}, we know that $\lambda_l$, $\bm{u}_l$ and $\bm{w}_l$ are all real-valued. 
Without loss of generality, assume that $\|\bm{a}\|_2 = 1$ and that $\bm{u}_l^{\star \top} \bm{u}_l>0$, which combined with Lemma \ref{lem:basic-uR-uL-rankr} yield
%
\begin{equation}
\bm{u}_l^\top \bm{u}_l^\star = 1 - o(1), \quad \bm{w}_l^\top \bm{u}_l^\star = 1- o(1), \quad \bm{w}_l^\top \bm{u}_l = 1 - o(1).
\end{equation}
%


The proof mainly follows the arguments employed in the analysis for the rank-1 case (cf.~Appendix~\ref{sec:proof-thm-distribution-validity}), with only a small number of changes needed. For the sake of brevity, we shall only point out the parts that require modifications. When we quote an argument in Appendix~\ref{sec:proof-thm-distribution-validity}, it is understood that we shall replace $\bm{u}$, $\bm{w}$, $\lambda$, $\cdots$ with $\ur_l$, $\ul_l$, $\lambda_l$, $\cdots$, respectively.  In addition, we note that 
%
\begin{equation}
	v_{\bm{a},l}^{\star} ~\asymp~ \sigma_{\max}^2  \,/\, ( \lambda_l^{\star} )^2 , 
\end{equation}
%
a consequence of Lemma~\ref{lem:va-properties} (or the relation \eqref{eq:va-bounds-simple}). 
%
\begin{enumerate}
	\item To begin with, the proof is built upon a sort of ``first-order'' approximation similar to \eqref{eq:au-approximation-3} in Lemma \ref{lemma:validity-auR-auL}. The validity of such an approximation in the rank-$r$ case requires additional conditions on the size of $\bm{a}^\top \bm{u}_k^\star$, as asserted below. The proof is deferred to Appendix~\ref{sec:proof-lemma:au-distribution-rankr}. 
%
\begin{lemma} 
\label{lem:au-distribution-rankr} 
Fix any unit vector $\bm{a} \in \mathbb{R}^n$, and assume that 
%
\begin{align}
|\bm{a}^{\top}\bm{u}_{k}^{\star}|  &=o\left(\frac{|\lambda_{l}^{\star}-\lambda_{k}^{\star}|}{|\lambda_{l}^{\star}|\sqrt{\mu\kappa^{4}r^{3}\log n}}\right),
  \qquad \forall k\neq l.  
\end{align}
%
Then under Assumption $\ref{assumption:noise-size-rankr}$, one has --- with probability $1 - O(n^{-6})$ --- that
%
\begin{align}
\label{eqn:coconut}
\left|\frac{\lambda_{l}}{\lambda_{l}^{\star}(\bm{u}_{l}^{\star\top}\bm{u}_{l})}\bm{a}^{\top}\bm{u}_{l}-\bm{a}^{\top}\bm{u}_{l}^{\star}-\frac{\bm{a}^{\top}\bm{H}\bm{u}_{l}^{\star}}{\lambda_{l}^{\star}}\right|=o\left(\frac{\sigma_{\max}}{|\lambda_{l}^{\star}|}\right) .
\end{align}	
%

In addition, if we further have $|\bm{a}^{\top}\bm{u}_{l}^{\star}|  =o(1/{\sqrt{\mu\kappa^{2}r^{4}\log n}})$, 
then with probability $1 - O(n^{-6})$, 
%
\begin{align}
\begin{cases}
\frac{1}{\bm{u}_l^{\star \top} \bm{u}_l} \bm{a}^\top \bm{u}_l = \bm{a}^\top \bm{u}_l^\star + \frac{\bm{a}^\top \bm{H} \bm{u}_l^\star}{\lambda_l^\star} + o \left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^\star|} \right) ; \\
\frac{1}{\bm{u}_l^{\star \top} \bm{w}_l} \bm{a}^\top \bm{w}_l = \bm{a}^\top \bm{u}_l^\star + \frac{\bm{a}^\top \bm{H}^\top \bm{u}_l^\star}{\lambda_l^\star} + o \left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^\star|} \right) .
\end{cases}
\end{align}
%
\end{lemma}


	\item Regarding the case when $|\bm{a}^{\top}\bm{u}^{\star}_l|\lesssim  \frac{\sigma_{\max} \sqrt{\log n}} { |\lambda_l^{\star}| } \asymp \sqrt{ v_{\bm{a},l}^{\star} \log n }$, the proof is exactly the same as the analysis in Appendix \ref{sec:small-norm-case-rank1}  (with Lemma \ref{lem:au-distribution-rankr} in place), and is hence omitted. 

	\item We now turn to the case when $|\bm{a}^{\top}\bm{u}^{\star}_l|\gtrsim \frac{\sigma_{\max} \sqrt{\log n} }{ |\lambda_l^{\star}| } \asymp \sqrt{ v_{\bm{a},l}^{\star} \log n }$, and assume without loss generality that $\bm{a}^{\top} \ur^{\star}_l>0$. Invoking Lemma  \ref{lem:au-distribution-rankr} and repeating the same argument in Appendix \ref{sec:large-norm-case-rank1}, we obtain
%
\begin{equation}
\frac{1}{\bm{u}_l^{\star \top} \bm{u}_l} \bm{a}^\top \bm{u}_l \cdot \frac{1}{\bm{u}_l^{\star \top} \bm{w}_l} \bm{a}^\top \bm{w}_l = \left(\bm{a}^\top \bm{u}^\star_l + \frac{\bm{a}^\top \left(\bm{H} + \bm{H}^\top \right) \bm{u}_l^\star}{2 \lambda_l^\star } + o\left(\frac{\sigma_{\mathrm{max}}}{\lambda_{\mathrm{min}}^\star} \right)\right)^2 . 
\end{equation}
%
The only remaining step then boils down to showing a result similar to \eqref{eq:diff-new-old} in Lemma \ref{LemCommonplace}, which helps eliminate the unknown information $\bm{u}_i^\star$ from our estimator. This is stated in the following lemma. 
%
\begin{lemma}
\label{lemma:uw-diff-rankr} 
Instate the assumptions of Lemma \ref{lem:au-distribution-rankr}. Suppose that $|\bm{a}^{\top}\bm{u}^{\star}_l|\gg \frac{\sigma_{\max} \sqrt{\log n} }{ |\lambda_l^{\star}| }$.  If 
$\big|\bm{a}^{\top}\bm{u}_{l}^{\star}\big|=o\left(1/\sqrt{\mu\kappa^{2}r^{4}\log n}\right)$ and $\big|\bm{a}^{\top}\bm{u}_{l}^{\star}\big|=o\left(\frac{\Delta_{l}^{\star}}{|\lambda_{l}^{\star}|\sqrt{\mu\kappa^{6}r^{3}\log n}}\right)$, then with probability at least $1-O(n^{-6})$, 
%
\begin{equation}
	\sqrt{\frac{1}{\bm{u}_{l}^{\top}\bm{w}_{l}}\bm{a}^{\top}\bm{u}_{l}\cdot\bm{a}^{\top}\bm{w}_{l}}-\sqrt{\frac{1}{\bm{u}_{l}^{\star\top}\bm{u}_{l}}\bm{a}^{\top}\bm{u}_{l}\cdot\frac{1}{\bm{u}_{l}^{\star\top}\bm{w}_{l}}\bm{a}^{\top}\bm{w}_{l}}=o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right).	
\end{equation}
%	
\end{lemma}

\end{enumerate}

\noindent With the above pieces in place, invoking the arguments presented for the rank-1 case (cf.~Appendix \ref{sec:proof-thm-distribution-validity}) immediately establishes Theorem~\ref{thm:distribution-validity-rankr}. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	

\subsubsection{Proof of Lemma \ref{lemma:uw-diff-rankr}}
	Apply the Neumann series again to otbain
	%
	\begin{align}
\bm{u}_{l} & =\sum_{k=1}^{r}\frac{\lambda_{k}^{\star}(\bm{u}_{k}^{\star\top}\bm{u}_{l})}{\lambda_{l}}\left\{ \sum_{s=0}^{\infty}\frac{1}{\lambda_{l}^{s}}\bm{H}^{s}\bm{u}_{k}^{\star}\right\} ;\\
\bm{w}_{l} & =\sum_{k=1}^{r}\frac{\lambda_{k}^{\star}(\bm{u}_{k}^{\star\top}\bm{w}_{l})}{\lambda_{l}}\left\{ \sum_{s=0}^{\infty}\frac{1}{\lambda_{l}^{s}}\left(\bm{H}^{\top}\right)^{s}\bm{u}_{k}^{\star}\right\} .
	\end{align}
	%
	Using such expansions and repeating the analysis in \eqref{eq:sushi} and \eqref{eq:T1-UB1}, we can express the inner product of them as
	%
	\begin{equation}
\bm{w}_{l}^{\top}\bm{u}_{l}=\sum_{k=1}^{r}\sum_{j=1}^{r}\frac{\lambda_{k}^{\star}\lambda_{j}^{\star}}{\lambda_{l}^{2}}\left(\bm{u}_{k}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{j}^{\star\top}\bm{w}_{l}\right)\left\{ 1+\frac{2}{\lambda_{l}}\bm{u}_{j}^{\star\top}\bm{H}\bm{u}_{k}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{ |\lambda_{l}^{\star}| } \right)\right\} .	
	\label{eq:wl-ul-prod-expansion}
	\end{equation}
	%

%Repeating the analysis in \eqref{eq:sushi} and \eqref{eq:T1-UB1}, 


	%
	In addition, for every pair $(k, j) \neq (l, l)$, Theorem \ref{thm:rankr-bounds} implies that
% 	\begin{equation}
% \left(\bm{u}_{k}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{j}^{\star\top}\bm{u}_{l}\right)=O\left(\frac{\sigma_{\mathrm{max}}}{\delta_{l}^{\star}}\sqrt{\mu\kappa^{4}r\log n}\right),
% 	\end{equation}
	%
	\begin{align}
\left(\bm{u}_{k}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{j}^{\star\top}\bm{u}_{l}\right)=\begin{cases}
O\left(\frac{\sigma_{\mathrm{max}}}{\Delta_{l}^{\star}}\sqrt{\mu\kappa^{4}r\log n}\right), & \text{if }k=l,j\neq l\text{ or }k\neq l,j=l,\\
O\left(\frac{\sigma_{\mathrm{max}}^{2}}{(\Delta_{l}^{\star})^{2}}\mu\kappa^{4}r\log n\right), & \text{if }k\neq l,j\neq l, 
\end{cases}
	\end{align}
	%
	thus indicating that
	%
\begin{align*}
\left|\sum_{k\neq l}\sum_{j\neq l}\frac{\lambda_{k}^{\star}\lambda_{j}^{\star}}{\lambda_{l}^{2}}\left(\bm{u}_{k}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{j}^{\star\top}\bm{w}_{l}\right)\left\{ 1+\frac{2}{\lambda_{l}}\bm{u}_{j}^{\star\top}\bm{H}\bm{u}_{k}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right)\right\} \right| & \lesssim r^{2}\kappa^{2}\max_{k\neq l,j\neq l}\big|\bm{u}_{k}^{\star\top}\bm{u}_{l}\big|\cdot\big|\bm{u}_{j}^{\star\top}\bm{w}_{l}\big|\\
 & \lesssim \left( \frac{\sigma_{\mathrm{max}}}{\Delta_{l}^{\star}}\sqrt{\mu\kappa^{6}r^{3}\log n} \right)^2 ;\\
\left|\sum_{j:j\neq l}\frac{\lambda_{l}^{\star}\lambda_{j}^{\star}}{\lambda_{l}^{2}}\left(\bm{u}_{l}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{j}^{\star\top}\bm{w}_{l}\right)\left\{ 1+\frac{2}{\lambda_{l}}\bm{u}_{j}^{\star\top}\bm{H}\bm{u}_{l}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right)\right\} \right| & \lesssim r\kappa\max_{j\neq l}\big|\bm{u}_{j}^{\star\top}\bm{w}_{l}\big|\lesssim\frac{\sigma_{\mathrm{max}}}{\Delta_{l}^{\star}}\sqrt{\mu\kappa^{6}r^{3}\log n};\\
\left|\sum_{k:k\neq l}\frac{\lambda_{k}^{\star}\lambda_{l}^{\star}}{\lambda_{l}^{2}}\left(\bm{u}_{k}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{l}^{\star\top}\bm{w}_{l}\right)\left\{ 1+\frac{2}{\lambda_{l}}\bm{u}_{l}^{\star\top}\bm{H}\bm{u}_{k}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right)\right\} \right| & \lesssim
	\frac{\sigma_{\mathrm{max}}}{\Delta_{l}^{\star}}\sqrt{\mu\kappa^{6}r^{3}\log n}.
\end{align*}
	% 
	These bounds taken together with \eqref{eq:wl-ul-prod-expansion} demonstrate that
	%
\begin{align}
\bm{w}_{l}^{\top}\bm{u}_{l} & =\frac{(\lambda_{l}^{\star})^{2}}{\lambda_{l}^{2}}\left(\bm{u}_{l}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{l}^{\star\top}\bm{w}_{l}\right)\left\{ 1+\frac{2}{\lambda_{l}}\bm{u}_{j}^{\star\top}\bm{H}\bm{u}_{k}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right)\right\} +O\left(\frac{\sigma_{\mathrm{max}}}{\Delta_{l}^{\star}}\sqrt{\mu\kappa^{6}r^{3}\log n}\right), 
	\label{eq:wl-ul-prod-expansion-2}
\end{align}
	%
	provided that $\sigma_{\mathrm{max}}\sqrt{\mu\kappa^{6}r^{3}\log n}\lesssim\Delta_{l}^{\star}$.  

	%
	Next, we have learned from Theorem~\ref{thm:eigengap-condition} and Lemma~\ref{lem:aHu-UB} that
	%
	\begin{align}
\left|\frac{\lambda_{l}-\lambda_{l}^{\star}}{\lambda_{l}}\right| & \lesssim \frac{\sigma_{\mathrm{max}}\sqrt{\mu\kappa^{2}r^{4}\log n}}{|\lambda_{l}^{\star}|} ,\\
%\lesssim???\lesssim\frac{\sigma_{\mathrm{max}}}{\delta_{i}^{\star}}\sqrt{\mu\kappa^{4}r^{5}\log n},\\
|\bm{u}_{l}^{\star\top}\bm{H}\bm{u}_{l}^{\star}| & \lesssim\sigma_{\mathrm{max}}\sqrt{\log n},
	\end{align}
	%
	which further lead to
	%
\begin{align*}
\left|\left(\bm{u}_{l}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{l}^{\star\top}\bm{w}_{l}\right)\left\{ \frac{2}{\lambda_{l}}\bm{u}_{j}^{\star\top}\bm{H}\bm{u}_{k}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right)\right\} \right| & \lesssim\frac{\sigma_{\mathrm{max}}\sqrt{\log n}}{|\lambda_{l}^{\star}|}\\
\left|\frac{(\lambda_{l}^{\star})^{2}}{\lambda_{l}^{2}}-1\right|\left|\left(\bm{u}_{l}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{l}^{\star\top}\bm{w}_{l}\right)\left\{ 1+\frac{2}{\lambda_{l}}\bm{u}_{j}^{\star\top}\bm{H}\bm{u}_{k}^{\star}+o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right)\right\} \right| & \lesssim\big|\lambda_{l}^{\star}-\lambda_{l}\big|\lesssim\frac{\sigma_{\mathrm{max}}\sqrt{\mu\kappa^{2}r^{4}\log n}}{|\lambda_{l}^{\star}|} .
\end{align*}
	%
	Substituting them into \eqref{eq:wl-ul-prod-expansion-2} and invoking the triangle inequality, we arrive at
	%
	\begin{align}
\bm{w}_{l}^{\top}\bm{u}_{l}=\left(\bm{u}_{l}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{l}^{\star\top}\bm{w}_{l}\right)+O\left(\frac{\sigma_{\mathrm{max}}\sqrt{\mu\kappa^{2}r^{4}\log n}}{|\lambda_{l}^{\star}|}+\frac{\sigma_{\mathrm{max}}}{\Delta_{l}^{\star}}\sqrt{\mu\kappa^{6}r^{3}\log n}\right).
	\label{eq:wl-ul-approx-error}
	\end{align}		


	Now we are ready to establish our final result. To this end, recall our derivation in \eqref{eq:may-day} and the fact $\bm{a}^{\top}\ur_l\asymp \bm{a}^{\top}\ul_l\asymp \bm{a}^{\top}\bm{u}^{\star}_l$. Thus, in order to ensure that
	\begin{equation}
\sqrt{\frac{1}{\bm{u}_{l}^{\top}\bm{w}_{l}}\bm{a}^{\top}\bm{u}_{l}\cdot\bm{a}^{\top}\bm{w}_{l}}-\sqrt{\frac{1}{\bm{u}_{l}^{\star\top}\bm{u}_{l}}\bm{a}^{\top}\bm{u}_{l}\cdot\frac{1}{\bm{u}_{l}^{\star\top}\bm{w}_{l}}\bm{a}^{\top}\bm{w}_{l}}=o\left(\frac{\sigma_{\mathrm{max}}}{ |\lambda_{l}^{\star} | }\right),	
	\end{equation}
	%
	it would suffice to show that
	%
	\begin{align}
\big|\bm{a}^{\top}\bm{u}_{l}^{\star}\big|\cdot\left|\bm{w}_{l}^{\top}\bm{u}_{l}-\left(\bm{u}_{l}^{\star\top}\bm{u}_{l}\right)\left(\bm{u}_{l}^{\star\top}\bm{w}_{l}\right)\right|=o\left(\frac{\sigma_{\mathrm{max}}}{|\lambda_{l}^{\star}|}\right). 
	\end{align}
	%
	In view of \eqref{eq:wl-ul-approx-error}, the above condition would hold as long as $\big|\bm{a}^{\top}\bm{u}_{l}^{\star}\big|=o\left(1/\sqrt{\mu\kappa^{2}r^{4}\log n}\right)$ and $\big|\bm{a}^{\top}\bm{u}_{l}^{\star}\big|=o\left(\frac{\Delta_{l}^{\star}}{|\lambda_{l}^{\star}|\sqrt{\mu\kappa^{6}r^{3}\log n}}\right)$. This concludes the proof. 




==> proof_rankr_inference.tex <==
%\section{Proof for eigenvector and eigenvalue inference}
%\label{sec:proof-rank-r-inference-all}

%\input{proof-theorem-rankr-CI.tex}
%\input{proof-evalue-inference-rank-r.tex}
%\input{proof-evector-inference-rank-r.tex}



